Computational Concentration of Measure: Optimal Bounds, Reductions, and More

Product measures of dimension $n$ are known to be concentrated in Hamming distance: for any set $S$ in the product space of probability $\epsilon$, a random point in the space, with probability $1-\delta$, has a neighbor in $S$ that is different from the original point in only $O(\sqrt{n\ln(1/(\epsilon\delta))})$ coordinates. We obtain the tight computational version of this result, showing how given a random point and access to an $S$-membership oracle, we can find such a close point in polynomial time. This resolves an open question of [Mahloujifar and Mahmoody, ALT 2019]. As corollaries, we obtain polynomial-time poisoning and (in certain settings) evasion attacks against learning algorithms when the original vulnerabilities have any cryptographically non-negligible probability. We call our algorithm MUCIO ("MUltiplicative Conditional Influence Optimizer") since proceeding through the coordinates, it decides to change each coordinate of the given point based on a multiplicative version of the influence of that coordinate, where influence is computed conditioned on previously updated coordinates. We also define a new notion of algorithmic reduction between computational concentration of measure in different metric probability spaces. As an application, we get computational concentration of measure for high-dimensional Gaussian distributions under the $\ell_1$ metric. We prove several extensions to the results above: (1) Our computational concentration result is also true when the Hamming distance is weighted. (2) We obtain an algorithmic version of concentration around mean, more specifically, McDiarmid's inequality. (3) Our result generalizes to discrete random processes, and this leads to new tampering algorithms for collective coin tossing protocols. (4) We prove exponential lower bounds on the average running time of non-adaptive query algorithms.

==> oldProof.tex <==

\section{Proof Using Ideal Partial-Expectations Oracle}
The following result works in the ideal model in which the partial-expectations oracle $\fhat{\cdot}{}$ is available to the online tampering algorithm $\Tam$. Using this oracle, $\Tam$ will \emph{not} need to have oracle access to $f(\cdot)$ or an online sampler $\wDist[\cdot]$ for $\wDistVec$. \Snote{Don't we need an oracle for the maximum jump too?} \Mnote{you mean alpha? we are fixing it now, but we can comment in a remark that our proof extends to the version discussed in the intro and abstract.}

\begin{construction}[Online tampering using partial-expectations oracle $\fhat{\cdot}{}$] \label{const:tampBlock}
 Recall that we are given a prefix $\pfix{v}{i-1}$ that is finalized, and we are also given a candidate value $u_i$ for the $i$'th block (supposedly sampled from  $\wDist[\pfix{v}{i-1}]$) and we want to decide to keep $v_i=u_i$ or change it.
 Let $\lambda>0$ be a parameter of the attack to be chosen later, $v^*_i = \argmax_{y_i} \fhat{\pfix{v}{i-1},y_i}{}$ be the choice for $i$'th block that maximizes  $\fhat{\pfix{v}{i}}{}$, and let  $f^*=\fhat{\pfix{v}{i-1},v^*_i}{}$ be that maximum.
\begin{enumerate}
    \item (Case 1)  If $f^* \geq e^{\lambda \alpha_i} \cdot \fhat{\pfix{v}{i-1}}{}$, then output $v_i = v_i^*$ (regardless of $u_i$).
    \item (Case 2) Otherwise, if $\fhat{\pfix{v}{i-1},u_i}{}\leq e^{-\lambda \alpha_i} \cdot \fhat{\pfix{v}{i-1}}{} $ , then output $v_i = v_i^*$.
    \item (Case 3) Otherwise, keep the value $u_i$ and output $v_i = u_i$.
\end{enumerate}
\end{construction}

\begin{claim}[Average case analysis of  Construction \ref{const:tampBlock}] \label{clm:tampBlock} Let $\bfk_i$ be the Boolean random variable that $\bfk_i=1$ iff the tampering over the $i$'th block happens, and let  $\alk = \sum_{i \in [n]} \alpha_i \cdot \bfk_i$ capture  the resulting $\alHD$ distance between the jointly sampled $\uVec$ and $\vVec$. Then, it holds that
    $$\ln (1/\eps) \geq \Ex[\alk] \cdot \lambda - {\lambda^2  n}/{2}.$$
\end{claim}
\paragraph{Corollary of Claim \ref{clm:tampBlock}.} By choosing  $\lambda = \sqrt {2\ln (1/\eps) / n}$, we obtain $\Ex[\alk] \leq \sqrt{2n\ln(1/\eps)}$. 



\paragraph{}We prove the following stronger statement that implies Claim \ref{clm:tampBlock}.
\begin{claim} \label{clm:stronger}
Let $\pfix{v}{i-1}$ be fixed.  Then,
$$\ln (1/\fhat{v}{i-1}) - \Ex_{v_i \gets \vDist[ \pfix{v}{i-1}]}[\ln(1/\fhat{v}{i})] \geq \Pr[\bfk_i]  \cdot \alpha_i\cdot \lambda  -  {\alpha_i^2 \cdot \lambda^2}/{2}.$$
\end{claim}

\begin{proof}[Proof of Claim \ref{clm:tampBlock} using Claim \ref{clm:stronger}.] A key property of Construction \ref{const:tampBlock} is that, because the tampering algorithm does not allow the function reach $0$, the final sequence $\vVec$ always makes the function $1$, namely
\begin{equation} \label{eq:always1}
    \Pr[f(\pfix{\vDist}{n})=1]=1.
\end{equation} Using the above equation, Claim \ref{clm:tampBlock} follows from Claim \ref{clm:stronger} and linearity of expectation as follows.
\begin{align*}
    \ln (1/\eps) &= \ln (1/\fhat{\es}{}) - \Ex[\ln (1)]  \\
    \text{(by Equation \ref{eq:always1})}~~~~ &= \ln (1/\fhat{\es}{}) - \Ex[\ln (1/\fhat{\vDist}{n})] \\
    \text{(by linearity of expectation)}~~~~ &= \sum_{i \in [n]} \left[\Ex[\ln (1/\fhat{\vDist}{i-1}) - \Ex[\ln (1/\fhat{\vDist}{i})]\right] \\
    \text{(by Claim \ref{clm:stronger})}~~~~ &\geq \sum_{i \in [n]} \left[ \Ex[\alpha_i\cdot \bfk_i] \cdot \lambda  - \frac{ \alpha_i^2\cdot \lambda^2}{2}\right] \\
    \text{(by linearity of expectation)}~~~~ &= \Ex[\alk] \cdot \lambda - \frac{n\cdot\lambda^2}{2}.
\end{align*}

\end{proof}

In the following, we will focus on proving Claim \ref{clm:stronger}.

\begin{proof}[Proof of  Claim \ref{clm:stronger}]
 There are 2 cases for a fixed $\pfix{v}{i-1}$:
\begin{itemize}
    \item If tampering of Case 1 happens, then we have $\Pr[\bfk_i=1]=1$, and 
    $$ \ln (1/\fhat{v}{i-1}) - \Ex_{v_i \gets (\vDist[ \pfix{v}{i-1}]}[\ln(1/\fhat{v}{i})]  = \ln (1/\fhat{v}{i-1})  - \ln (1/f^*)  \geq \lambda \alpha_i.$$ 
    Thus, in this case Claim \ref{clm:stronger} follows trivially.
    \item If tampering of Case 1 does not happen, it means that $f^* = \sup_{y_i} \fhat{\pfix{u}{i-1},y_i}{}$  is bounded from above. In the following, we focus on this case and all the probabilities and expectations are conditioned on Case 1 not happening; namely, that .
\end{itemize}

Let $I(\pfix{v}{i})$ be the indicator function for the set $\set{\pfix{v}{i}\colon {\fhat{v}{i}} \leq e^{-\lambda \alpha_i}\cdot{\fhat{v}{i-1}}}.$ We have
$$\Pr_{(u_i,v_i) \gets (\wDist,\vDist)[\pfix{v}{i-1}]}\left[\fhat{v}{i} \geq \max\left(e^{-\lambda \alpha_i}\cdot \fhat{v}{i-1},\fhat{\pfix{v}{i-1},u_i}{}\right)\cdot e^{\lambda \alpha_i\cdot I(\pfix{v}{i-1},u_i)} \right] = 1.$$

Note that the two terms on each side of the inequality inside the probability above depend only on either of $u_i$ or $v_i$ (not both). Therefore, by sampling them separately, and  by linearity of expectation  we have

 \begin{align*}
 &\Ex_{v_i \gets \vDist[\pfix{v}{i-1}]}[\ln(\fhat{v}{i})]\\
 &\geq \Ex_{u_i \gets \wDist[\pfix{v}{i-1}]}\left[\ln\left(\max\left(e^{-\lambda\alpha_i}\cdot \fhat{v}{i-1},\fhat{\pfix{v}{i-1},u_i}{}\right)\cdot e^{\lambda\cdot\alpha_i\cdot I(\pfix{v}{i-1},u_i)}\right) \right]\\
 &= \Ex_{u_i \gets \wDist[\pfix{v}{i-1}]}\left[\ln\left(\max\left(e^{-\lambda\alpha_i}\cdot \fhat{v}{i-1},\fhat{\pfix{v}{i-1},u_i}{}\right)\right)\right] + \lambda\cdot\alpha_i \cdot \Ex_{u_i \gets \wDist[\pfix{v}{i-1}]}[ I(\pfix{v}{i-1},u_i) ]\\
 &= \Ex_{u_i \gets \wDist[\pfix{v}{i-1}]}\left[\ln\left(\max\left(e^{-\lambda\alpha_i}\cdot \fhat{v}{i-1},\fhat{\pfix{v}{i-1},u_i}{}\right)\right)\right] + \lambda\cdot\alpha_i \cdot \Ex[\bfk_i]. \stepcounter{equation}\tag{\theequation}\label{ineq:01}
 \end{align*}
Now, for a fixed $\pfix{v}{i-1}$, consider the random variable $\bft$ defined as follows $$\bft\equiv\frac{ \max\left(e^{-\lambda\cdot \alpha_i}\cdot \fhat{v}{i-1},\fhat{\pfix{v}{i-1},\wDist[\pfix{v}{i-1}]}{}\right)}{\fhat{v}{i-1}}.$$
It holds that
$$\Pr\left[e^{-\lambda\alpha_i}\leq \bft \leq e^{\lambda\alpha_i}\right]=1.$$
It also holds that
$$\Ex\left[\bft\cdot \fhat{v}{i-1}\right] = \Ex \left[\max\left(e^{-\lambda}\cdot \fhat{v}{i-1},\fhat{\pfix{v}{i-1},\wDist[\pfix{v}{i-1}]}{}\right)\right] \geq \fhat{v}{i-1}$$
which implies $\Ex[\bft] \geq 1$. Now using Lemma \ref{lemma:numerical} we have  $\Ex[\ln(\bft)] \geq -\frac{\lambda^2\cdot \alpha_i^2}{2}$ which implies 
\begin{align*}\Ex\left[\ln\left(\max\left(e^{-\lambda\alpha_i}\cdot \fhat{v}{i-1},\fhat{\pfix{v}{i-1}, \wDist[\pfix{v}{i-1}]}{}\right)\right)\right] \geq \ln(\fhat{v}{i-1}) - \frac{\lambda^2\alpha_i^2}{2}.\stepcounter{equation}\tag{\theequation}\label{ineq:02}
\end{align*}
 Combining Equations (\ref{ineq:01}) and (\ref{ineq:02}), we get
 $$\Ex_{v_i \gets \vDist[\pfix{v}{i-1}]}\left[\ln(\fhat{v}{i})\right]  \geq \ln(\fhat{v}{i-1}) + \lambda\cdot\alpha_i \cdot \Ex[\bfk_i] - \frac{\lambda^2\cdot \alpha_i^2}{2}$$
 which finishes the proof of   Claim \ref{clm:stronger}.
\end{proof}

\subsection{Tampering  with Abort}

\begin{construction}[Online tampering \emph{with abort} $\TamAb$ using  partial-expectations oracle] \label{const:tampBlockAbort} This construction is identical to Construction \ref{const:tampBlock}, except that whenever the  fixed prefix has a too small partial expectation $\fhat{\pfix{v}{i-1},u_i}{}$ (based on a new parameter $\tau$) we will abort. Also, in that case the tampering algorithm does not tamper with any future $v_i$ block either. Namely, we add the following ``Case 0'' to the previous steps:
\remove{
 Recall that we are given a prefix $\pfix{v}{i-1}$ that is finalized, and we are also given a candidate value $u_i$ for the $i\th$ block (supposed sampled from the distribution $\wDist[\pfix{v}{i-1}]$ and we want to decide to keep $v_i=u_i$ or change it.
 Let $\lambda>0$ be a parameter of the attack to be chosen later, $v^*_i = \argmax_{y_i} \fhat{\pfix{v}{i-1},y_i}{}$ be the choice for $i\th$ block that maximizes  $\fhat{\pfix{v}{i}}{}$, and  $f^*=\fhat{\pfix{v}{i-1},v^*_i}{}$.
 }
\begin{itemize}
%\setcounter{enumi}{-1}
\item (Case 0) If $\fhat{\pfix{v}{i-1},u_i}{}\leq e^{-\tau}\cdot \eps$ abort. If had aborted before, do nothing. 
\remove{
    \item (Case 1)  Otherwise, if $f^* \geq e^{\lambda \alpha_i} \cdot \fhat{\pfix{v}{i-1}}{}$, then output $v_i = v_i^*$ (regardless of $u_i$).
    \item (Case 2) Otherwise, if $\fhat{\pfix{v}{i-1},u_i}{}\leq e^{-\lambda \alpha_i} \cdot \fhat{\pfix{v}{i-1}}{} $ , then output $v_i = v_i^*$.
    \item (Case 3) Otherwise, keep the value $u_i$ and output $v_i = u_i$.
}
\end{itemize}
\end{construction}

\remove{
\begin{claim}[Average case analysis of  Construction \ref{const:tampBlockAbort}] \label{clm:tampBlockAbort} Let $\bfk_i$ be the Boolean random variable that captures if tampering over the $i\th$ block happens or not, and let  $\alk = \sum_{i \in [n]} \alpha_i \cdot \bfk_i$. Then, 
    $$\ln (1/\eps) \geq \Ex[\alk] \cdot \lambda - \frac{\lambda^2 \cdot n}{2}.$$
\end{claim}
}

\paragraph{Average case analysis of  Construction \ref{const:tampBlockAbort}.} The average number of tampering of Construction \ref{const:tampBlockAbort} is trivially less than average number of tampering of Construction \ref{const:tampBlock}. Therefore, the same bound of Claim \ref{clm:tampBlock} still applies to Construction \ref{const:tampBlockAbort} as well.

\begin{claim} The probability of ever aborting during sampling 
$(\uVec,\vVec)\gets \jointSamp{\wDistVec}{\TamAb}$  
is at most $e^{-\frac{(\tau - n\cdot\lambda^2/2)^2}{2\cdot n\cdot \lambda^2}}$. As a result,  for $\delta=n\cdot e^{-\frac{(\tau - n\cdot\lambda^2/2)^2}{2\cdot n\cdot \lambda^2}}$ (i.e., choosing $\tau= \ln(\nicefrac{1}{\eps}) + \sqrt{4\ln(\nicefrac{\delta}{n})\cdot\ln(\nicefrac{1}{\eps})}$) we also have
$$\Ex_{(\uVec,\vVec)\gets \jointSamp{\wDistVec}{\TamAb}}[f(\vVec)] \geq 1 - \delta.$$ 
\end{claim}
\begin{proof}
Define $f^*(\pfix{v}{i-1}) = \max_{y_i}\fhat{\pfix{v}{i-1}, y_i}{}$. We also define Boolean indicator functions $I_0, I_1, I_2$ and $I_3$, as well as a real-valued vector $\yVec$  as follows.
The first function $I_0$ indicates that we have not aborted yet, and the others define a condition for their corresponding cases in Constructions \ref{const:tampBlock} and \ref{const:tampBlock}.
$$I_0(\pfix{v}{i-1}) = \begin{cases}
0 & \text{if $\forall j\leq i;~\fhat{v}{j} \geq \eps\cdot e^{-\tau}$,}\\
1 & \text{otherwise.}\\
\end{cases}$$
%The second function, captures the Case 1 of the construction \ref{const:tampBlockAbort}.
$$I_1(\pfix{v}{i-1})= \begin{cases}
1 & \text{if $f^*(\pfix{v}{i-1}) \geq e^{\lambda\cdot \alpha_i}\cdot\fhat{v}{i-1}$ and $\neg I_0(\pfix{v}{i-1})$},\\
0 & \text{otherwise;}\\
\end{cases}$$
%The third function, captures the Case 2 of the construction \ref{const:tampBlockAbort}.
$$I_2(\pfix{v}{i}) =\begin{cases}
1 & \text{if $\fhat{v}{i} \leq e^{-\lambda\cdot \alpha_i}\cdot\fhat{v}{i-1}$ and $\neg I_1(\pfix{v}{i-1})$ and $\neg I_0(\pfix{v}{i-1})$},\\
0 & \text{otherwise;}\\
\end{cases}
$$
The last function indicates that the above conditions are \emph{not} happening.
$$I_3(\pfix{v}{i})=\begin{cases}
1 & \text{if $\neg I_0(\pfix{v}{i})$ and $\neg I_1(\pfix{v}{i-1})$ and $\neg I_2(\pfix{v}{i})$},\\
0 & \text{otherwise.}\\
\end{cases}$$



Finally, we define a real-valued function $y$ as follows that captures the change in the potential function for the cases where none of $I_0,I_1,I_2$ are happening.
$$y(\pfix{v}{i}) = \left(\ln(\fhat{v}{i}) - \ln(\fhat{v}{i-1})\right)\cdot I_3(\pfix{v}{i}).$$
Now consider a sequence of random variables $\yDistVec = (\yDist_1,\dots,\yDist_n)$ sampled as follows. We first sample $(\uVec, \vVec )\gets (\uDistVec, \vDistVec)$ then set $y_i= y(\pfix{v}{i-1}, u_i) = y(\pfix{v}{i})$ for $i \in [n]$. Note that $y(\pfix{v}{i-1}, u_i) = y(\pfix{v}{i})$ because if $I_3(\pfix{v}{i-1}, u_i) = 1$ it means that $u_i = v_i$.
\begin{claim}\label{clm:submart1}
We have $\Ex[e^{\yDist_i} \mid \pfix{y}{i-1}] \geq 1$.
\end{claim}
\paragraph{Notation.} Since $I_j(\cdot)$'s are Boolean, we can use the notation $(I_i \lor I_j)(\pfix{v}{i})$ or $(1- (I_i \lor I_j))(\pfix{v}{i})$ based on logical operators to construct more Boolean indicators.
\begin{proof}[Proof of Claim \ref{clm:submart1}] \Mnote{Better to first say in English, informally, why this is the case. + fix left right paranthesis + you might say in english that we prove something stronger that conditions on vi (which determines yi) and then the calculation below is also a bit more clear and simpler}
\begin{align*}
\Ex[e^{\yDist_i}\mid\pfix{y}{i-1}] &= \Ex_{\pfix{v}{i-1} \gets (\pfix{\vDist}{i-1} \mid \pfix{y}{i-1})}\left[\Ex_{u_i \gets \wDist[\pfix{v}{i-1}]}\left[e^{\left(\ln(\fhat{\pfix{v}{i-1},u_i}{}) - \ln(\fhat{v}{i-1})\right)\cdot I_3(\pfix{v}{i-1},u_i)}\right]\right]\\
&\geq\Ex_{\pfix{v}{i-1} \gets (\pfix{\vDist}{i-1} \mid \pfix{y}{i-1})}\left[\Ex_{u_i \gets \wDist[\pfix{v}{i-1}]}\left[e^{\left(\ln(\fhat{\pfix{v}{i-1},u_i}{}) - \ln(\fhat{v}{i-1})\right)\cdot \left((I_3 \lor I_2)\left(\pfix{v}{i-1},u_i\right)\right)}\right]\right]\\
&= \Ex_{\pfix{v}{i-1} \gets (\pfix{\vDist}{i-1} \mid \pfix{y}{i-1})}\left[\Ex_{u_i \gets \wDist[\pfix{v}{i-1}]}\left[e^{\left(\ln(\fhat{\pfix{v}{i-1},u_i}{}) - \ln(\fhat{v}{i-1})\right)\cdot \left(1-(I_1 \lor I_0)\left(\pfix{v}{i-1}\right)\right)}\right]\right]\\
&\geq \Ex_{\pfix{v}{i-1} \gets (\pfix{\vDist}{i-1} \mid \pfix{y}{i-1})}\left[\min(\Ex_{u_i \gets \wDist[\pfix{v}{i-1}]}\left[e^{\left(\ln(\fhat{\pfix{v}{i-1},u_i}{}) - \ln(\fhat{v}{i-1})\right)}\right], 1)\right]\\
&= \Ex_{\pfix{v}{i-1} \gets (\pfix{\vDist}{i-1} \mid \pfix{y}{i-1})} \left[\min(\Ex_{u_i \gets \wDist[\pfix{v}{i-1}]}\left[\fhat{\pfix{v}{i-1},u_i}{}/\fhat{v}{i-1}\right],1)\right]\\
&= 1.
\end{align*}
\end{proof}

\begin{claim}\label{clm:tbounded}
We have $|y(\pfix{v}{i})| \leq \lambda\cdot \alpha_i$
\end{claim}
\begin{proof}
This follows from  the definition of $I_3$. If $I_3(\pfix{v}{i}) = 1$ it means that $e^{-\lambda\cdot \alpha_i}\cdot \fhat{v}{i-1}\leq \fhat{v}{i} \leq e^{-\lambda\cdot \alpha_i}\cdot\fhat{v}{i-1}$ and if $I_3(\pfix{v}{i})=0$ then $y(\pfix{v}{i})=0$. 
\end{proof}
\begin{claim}\label{clm:submart2}
We have $\Ex[\yDist_i \mid \pfix{y}{i-1}] \geq -\frac{\lambda^2\cdot\alpha_i^2}{2}$.
\end{claim}
\begin{proof}
The proof follows by using Lemma \ref{lemma:numerical} and Claims \ref{clm:submart1} and \ref{clm:tbounded}.
\end{proof}
\begin{claim}
The probability of aborting is at most 
$n\cdot e^{\frac{(\tau - \lambda n\cdot\lambda^2/2)^2}{2\cdot n\cdot \lambda^2}}.$
\end{claim}
\begin{proof}
By Claims \ref{clm:submart2} and \ref{clm:tbounded}, the sequence $\yDistVec = (\yDist_1,\dots,\yDist_n)$ forms an (approximate) submartingale and by Azuma inequality of Lemma \ref{lem:AzumaApp} we have,
$$\Pr\left[\sum_{i=1}^n \yDist_i \leq -\tau \right] \leq e^{-\frac{\left(\tau - n\cdot\lambda^2/2\right)^2}{2\cdot n\cdot \lambda^2}} ~~.$$
On the other hand, for every $\pfix{v}{i} \in \Supp(\pfix{\vDist}{i})$ we have 
$I_2(\pfix{v}{i}) = 0.$ Therefore, for every $\pfix{v}{j} \in \Supp(\pfix{\vDist}{j})$,
\begin{align*}
\ln(\fhat{v}{j}) &= \ln(\eps) + \sum_{i=1}^j (\ln(\fhat{v}{i})-\ln(\fhat{v}{i-1}))\\
 &= \ln(\eps) + \sum_{i=1}^j \left(\ln(\fhat{v}{i})-\ln(\fhat{v}{i-1})\right)\cdot\left((I_0\lor I_1)(\pfix{v}{i-1}) + I_3(\pfix{v}{i})\right)\\
 &\geq \ln(\eps) + \sum_{i=1}^j \left(\ln(\fhat{v}{i})-\ln(\fhat{v}{i-1})\right)\cdot\left(I_0(\pfix{v}{i-1}) + I_3(\pfix{v}{i})\right)\\
 &= \ln(\eps) + \sum_{i=1}^j y(\pfix{v}{i}) + \sum_{i=1}^j \left(\ln(\fhat{v}{i})-\ln(\fhat{v}{i-1})\right)\cdot I_0(\pfix{v}{i-1}).
\end{align*}
We now calculate probability of the event $A_j$ that the partial average goes bellow $e^{-\tau}\cdot \eps$ (i.e., abort happens)  at the $j\th$ block for the \emph{first time}.
\begin{align*}
    \Pr_{\pfix{v}{j} \gets \pfix{\vDist}{j}}[A_j] &= \Pr_{\pfix{v}{j} \gets \pfix{\vDist}{j}}\left[ \fhat{v}{j} \leq e^{-\tau}\cdot \eps \land \neg I_0(\pfix{v}{j-1})\right]\\
    &= \Pr_{\pfix{v}{j} \gets \pfix{\vDist}{j}}[ \ln(\fhat{v}{j}) \leq -\tau +\ln(\eps) \land \neg I_0(\pfix{v}{j-1})]\\
    &\leq \Pr_{\pfix{v}{j} \gets \pfix{\vDist}{j}}\left[\sum_{i=1}^j y(\pfix{v}{i}) + \sum_{i=1}^j \left(\ln(\fhat{v}{i})-\ln(\fhat{v}{i-1})\right)\cdot I_0(\pfix{v}{i-1}) \leq -\tau \land \neg I_0(\pfix{v}{j-1})\right]\\
   &\leq \Pr_{\pfix{v}{j} \gets \pfix{\vDist}{j}}\left[\sum_{i=1}^j y(\pfix{v}{i}) \leq -\tau\right] \\
   &\leq e^{-\frac{(\tau - n\cdot\lambda^2/2)^2}{2\cdot n\cdot \lambda^2}}.
\end{align*}
The above means that the probability that Construction \ref{const:tampBlockAbort} enters the abort state is less than $n\cdot e^{-\frac{(\tau - n\cdot\lambda^2/2)^2}{2\cdot n\cdot \lambda^2}}$. 
\end{proof}
We already know that if abort does not happen then the output will always be $1$. Therefore, we have
$$\Ex_{\vVec\gets \vDistVec}[f(\vVec)] \geq 1- n\cdot e^{-\frac{(\tau - n\cdot\lambda^2/2)^2}{2\cdot n\cdot \lambda^2}}.$$
Now, if we set $\tau = \ln(\nicefrac{1}{\eps}) + \sqrt{4\ln(\nicefrac{\delta}{n})\cdot\ln(\nicefrac{1}{\eps})}$ and $\lambda=\sqrt{-\ln(\eps)/n}$,  we get 
$$\Ex_{\vVec\gets \vDistVec}[f(\vVec)] \geq 1-\delta.$$
\end{proof}


